From Quasi-Dominions to Progress Measures

We revisit the approaches to the solution of parity games based on progress measures and show how the notion of quasi dominions can be integrated with those approaches. The idea is that, while progress measure based techniques typically focus on one of the two players, little information is gathered on the other player during the solution process. Adding quasi dominions provides additional information on this player that can be leveraged to greatly accelerate convergence to a progress measure. To accommodate quasi dominions, however, non trivial refinements of the approach are necessary. In particular, we need to introduce a novel notion of measure and a new method to prove correctness of the resulting solution technique.

==> SectionVI.tex <==

%%****************************************************************************%%
%%                                                                            %%
%% Article Title                                                              %%
%%                                                                            %%
%% SectionVI.tex                                                              %%
%%                                                                            %%
%% Revision 0                                                                 %%
%%                                                                            %%
%% Copyright (C) 20xx, Fabio Mogavero.                                        %%
%% All rights reserved.                                                       %%
%%                                                                            %%
%%****************************************************************************%%

% Begin of file SectionVI.tex

\begin{section}{...}
  \label{sec:vi}

  \cbstart
  ...
  \cbend


  \begin{subsubsection}{...}

    \cbstart
    ...
    \cbend

  \end{subsubsection}


  \begin{subsubsection}{...}

    \cbstart
    ...
    \cbend

  \end{subsubsection}


  \begin{subsubsection}{...}

    \cbstart
    ...
    \cbend

  \end{subsubsection}


  \begin{subsubsection}{...}

    \cbstart
    ...
    \cbend

  \end{subsubsection}

\end{section}

% End of file SectionVI.tex

